Programming interfaces and basic topology

A pattern of interaction that arises again and again in programming is a "handshake", in which two agents exchange data. The exchange is thought of as provision of a service. Each interaction is initiated by a specific agent--the client or Angel--and concluded by the other--the server or Demon. We present a category in which the objects--called interaction structures in the paper--serve as descriptions of services provided across such handshaken interfaces. The morphisms--called (general) simulations--model components that provide one such service, relying on another. The morphisms are relations between the underlying sets of the interaction structures. The proof that a relation is a simulation can serve (in principle) as an executable program, whose specification is that it provides the service described by its domain, given an implementation of the service described by its codomain. This category is then shown to coincide with the subcategory of "generated" basic topologies in Sambin's terminology, where a basic topology is given by a closure operator whose induced sup-lattice structure need not be distributive; and moreover, this operator is inductively generated from a basic cover relation. This coincidence provides topologists with a natural source of examples for non-distributive formal topology. It raises a number of questions of interest both for formal topology and programming. The extra structure needed to make such a basic topology into a real formal topology is then interpreted in the context of interaction structures.

==> localization.tex <==
%% master: main.tex



\subsubsection{Localization and distributivity}

The basic topology obtained from an interaction structure is not in general
distributive. One way to obtain distributivity is to add a condition of
\emph{convergence} (page~\pageref{convergence}).  In~\cite{induc_top}, the
authors introduce the notion of ``localized'' axiom set which gives rise to
convergent basic topologies, \ie~formal topologies.

If $w=<A,D,n>$ is an interaction structure, a preorder $\leq$ on $S$ is said to
be localized if the following holds:
\[
  s \leq s'\ ,\ a'\in A(s')
  \quad => \quad
  s |= w\Bigg( \bigcup_{d'\in D(s',a')} \SING{s'[a'/d']}  \BinDown
  \SING{s}\Bigg)
\]
This implies in particular that $\geq$ is a linear simulation.

\medbreak
Suppose that $\leq$ is localized; if we extend the generating rules with
\begin{center}
  \infer{s'|= U & s\leq s'}{s|=\A(U)}{$\leq$-compat}. \label{compat-rule}
\end{center}
then the resulting lattice is distributive: this is one of the results
of~\cite{induc_top}. (The rules were slightly more complex because they had
to consider the positivity predicate and the positivity axiom).
Note that since $\leq$ is a preorder ---and as such, reflexive--- this rule is
a generalization of the reflexivity rule.

\smallbreak
The preorder is intended to represent \textit{a priori} the notion of
inclusion between basic opens. The smallest interesting preorder to consider
is the following: ``$s_1 \leq s_2$ iff $s_1|=\A\{s_2\}$''. This preorder is
the saturation of the identity
%(which is itself the reflexive and transitive closure of the empty relation),
and it appears implicitly in the definition of convergence.


\medbreak
The rest of this section is devoted to an analysis of the notion of
localization in the context of interaction structures, together with a
tentative computational interpretation. It culminates with an interpretation
of the notion of formal points in terms of server programs.


\paragraph{Interaction structure with self-simulation.}

The first step is to add a preorder on states, and to require it to be
well-behaved with respect to its parent interaction structure.

\begin{defn}
  An interaction structure with \newterm{self-simulation} on $S$ is a pair $<w,R>$
  where
  \begin{itemize}
    \item $w$ is an interaction structure on $S$;
    \item $R$ is a general simulation from $w$ to itself.
  \end{itemize}
\end{defn}

\begin{lem}
If $R$ is a simulation from $w$ to itself, then so is the reflexive
transitive closure of $R$.
\end{lem}
\begin{proof}
  This is a direct consequence of the following facts: identities are
  simulations, simulations compose (proposition~\ref{prop:simCategory}) and
  simulations are closed under unions (proposition~\ref{prop:simClosedUnion}).

\end{proof}
As a result, we can always assume the self-simulation to be a preorder, and we
call it ``$\geq$''. The meaning of ``$s\leq s'$'' is thus ``$s$ simulates $s'$ in
$w$''.

\noindent
We have:
\begin{lem} \label{lem:downClosureCover}
  $s <| V$ implies $\downclosure{\{s\}} <| \downclosure{V}$.
\end{lem}
\begin{proof}
This is just an application of proposition~\ref{prop:linSimChar}.
\end{proof}


\smallbreak
Two extreme examples of such self simulations are:
\begin{itemize}
  \item the empty relation, or the identity (its reflexive/transitive
    closure).  This is isomorphic to the case of normal interaction structures.

  \item $R == (\J_w(S)×S) \cup (S×\A_w(\emptyset))$. The intuition is
    that $(s_D,s_A)|=R$ iff the Demon can avoid deadlocks from $s_D$ or the
    Angel can deadlock the Demon from $s_A$.\footnote{A deadlock is a state in
    a system in which it is impossible to do something.} Classically, this can
    be shown to be the biggest simulation (\ie~it is the union of all
    simulations) on an interaction structure and \textit{a~fortiori}, we have
    $R = \RTC{R} = \Sat{\RTC{R}}$.\footnote{Recall that classically,
    $\J_w(S)=\comp\A_w(\emptyset)$, which implies that
    $\comp R=\A_w(\emptyset)×\J_w(S)$.}
\end{itemize}
The second example shows that the possibility of driving the Demon into a
deadlock is the weakest property that ``needs to be respected'' by a self
simulation.

% removed (old)???
%\begin{remark}
%  In practice, a self simulation will lie strictly between those two.  A simple
%  example is following. Suppose we have a set of names ($x$, \ldots) for ``single-assignment'' variables,
%  \ie~variables that start in a special uninitialised state, and can be be assigned
%  (natural number) value at most once.  Let $S$ be the set of variable assignments, \ie~a state
%  $\rho \in S$ is a map from variable names to $\{\bot\}+\mathbb{N}$:
%  \begin{itemize}
%    \item if $\rho(x)=\bot$, then the variable $x$ is not initialized;
%    \item if $\rho(x)=n$, then the variable $x$ has the value $n$.
%  \end{itemize}
%  Suppose the Angel has the ability to initialize a variable, but not the
%  ability to change an existing value.  We can define $\rho_1\leq \rho_2 ==
%  (\forall x) \rho_1(x)\leq\rho_2(x)$ where the right ``$\leq$'' is the usual
%  ordering on the flat domain $\{\bot\}+\mathbb{N}$.
%\end{remark}



\paragraph{Interaction structures and localization.}

We now investigate the result of strengthening the condition to get full
localization.

\begin{defn} \label{defn:localized}
  Let $w$ be an interaction structure on $S$; a simulation preorder~$\geq$ on
  $S$ is localized if the following holds:
  \[
    s_1 \leq s_2\ ,\ a_2\in A(s_2)
    \quad => \quad
    s_1   <|_w  \bigcup_{d_2\in D(s_2,a_2)} \SING{s_2[a_2/d_2]}  \BinDown
    \SING{s_1}
    \ \hbox{.}
  \]
\end{defn}
\noindent
This condition is slightly more general than the one from~\cite{induc_top} in
the sense that it considers general simulations rather than linear ones.  Note
also that in contrast to the notion of convergence from
definition~\ref{def:convergence}, this definition doesn't require equality:
$\downclosure{\SING{s}}$ is defined in terms of $\leq$.

%%% removed (old) ???
%%% \smallbreak
%%% Here is a programming reading of the right hand side of this formula:
%%% ``$s$ can simulate $s'$ \emph{without losing knowledge of what is
%%% available in $s$}''. The reason is that the new state $s[a'/d']$ will
%%% simulate $s$, \ie~every finite sequence of interactions which was
%%% available from $s$ is still available from $s[a'/d']$. This intuition
%%% will be formally justified with lemma~\ref{lem:localized}.
\smallbreak
First, we need a lemma.

\begin{lem}
  Suppose $\geq$ is a localized preorder on $w$; then we have:
  \[
    s_1 \leq s_2\ ,\ a_2'\in \RTC{A}(s_2)
    \quad => \quad
    s_1   <|_w  \bigcup_{d_2'\in \RTC{D}(s_2,a_2')} \SING{s_2[a_2'/d_2']}  \BinDown
    \SING{s_1}
    \ \hbox{.}
  \]
\end{lem}
This means that the additional condition is well behaved with respect to the
RTC operation. (This is analogous to
point~\textit{\ref{lem:genSimChar:pt:RTC}} of lemma~\ref{lem:genSimChar}; and
indeed, the proof is very similar.)

\begin{proof}
Suppose that $s_1\leq s_2$ and let $a'_2\in \RTC{A}(s_2)$. We work by induction
on the structure of $a'_2$.

\begin{itemize}
\item if $a'_2 = \Exit$, this is trivial.

\item if $a'_2 = \Call(a_2,k_2)$: since $\geq$ is localized, we know that
  \[
    s_1 <| \bigcup_{d_2}\downclosure{\SING{s_2[a_2/d_2]}} \cap
                                     \downclosure{\SING{s_1}}
    \ \hbox{.}
  \]
  %
  Let $s'_1|= \bigcup_{d_2}\downclosure{\SING{s_2[a_2/d_2]}} \cap
  \downclosure{\SING{s_1}}$, in particular $s'_1\leq s_2[a_2/d_2]$ for some
  $d_2\in D_2(s_2,a_2)$. We can apply the induction hypothesis for $s'_1\leq
  s_2[a_2/d_2]$ and $k_2(d_2)$ to obtain:
  %
  \[
    s'_1
    \quad <|
    \bigcup_{d'_2\in \RTC{D}(s_2[a_2/d_2],k_2(d_2))}
      \downclosure{\SING{s_2[a_2/d_2]\big[k_2(d_2)/d_2'\big]}}
      \cap
      \downclosure{\{s'_1\}}
    \ \hbox{.}
  \]
  %
  We have
  $\bigcup_{d'_2\in \RTC{D}(s_2[a_2/d_2],k_2(d_2))}
  \sub
  \bigcup_{d'_2\in \RTC{D}(s_2,a_2')}$
  and $\downclosure{\SING{s_1'}}\sub\downclosure{\SING{s_1}}$
  (because $s_1'\leq s_1$).
  \\
  The RHS is thus included in $\bigcup_{d'_2\in
  \RTC{D}(s_2,a_2')}\downclosure{\SING{s_2[a_2'/d_2']}} \cap
  \downclosure{\SING{s_1}}$; and so, by monotonicity:
  %
  \[
    \bigcup_{d_2}\downclosure{\SING{n(s_2,a_2,d_2)}} \cap \downclosure{\SING{s_1}}
    \quad  <|
    \bigcup_{d'_2\in \RTC{D}(s_2,a_2')}\downclosure{\SING{s_2[a_2'/d_2']}} \cap
                                     \downclosure{\SING{s_1}}
    \ \hbox{.}
  \]
  We get the result by transitivity.
\end{itemize}
\end{proof}

\begin{lem}\label{lem:localized}
  Suppose $<w,\geq>$ is a localized interaction structure; then $s <| U$
  implies $s <| \downclosure{U}\cap \downclosure{\{s\}}$.
\end{lem}
\begin{proof}
  Let $s <| U$, \ie~$(\exists a')\,\bigcup_{d'}\SING{s[a'/d']}\sub U$.
  Since $\leq$ is reflexive, and by the previous lemma, we know that
  \[
    s <|
    \bigcup_{d'}\downclosure{\SING{\RTC{n}(s,a',d')}} \cap \downclosure{\SING{s}}
    \ \hbox{.}
  \]
  The RHS is obviously included in $\downclosure{U}\cap\downclosure{\{s\}}$,
  so we get the result by monotonicity.

\end{proof}


\begin{cor} \label{cor:coverDownclosure}
  If $U <| V$ then $U <| \downclosure{U} \cap \downclosure{V}$.
\end{cor}

We will now check that convergence is satisfied for such a $(S,\A_{w},\leq)$.
\begin{prop} \label{prop:localizedConvergent}
if $s <| U$ and $s <| V$, then $s <| \BinDown U\cap \BinDown V$.
\end{prop}
\begin{proof}
  By lemma~\ref{lem:localized}, we know that
  $s <| \downclosure{U}\cap \downclosure{\SING{s}}$.
  By lemma~\ref{lem:downClosureCover} we know that
  $\downclosure{\SING{s}} <| \downclosure V$, which implies
  $\downclosure U \cap \downclosure{\SING{s}} <| \downclosure V$;
  which (by corollary~\ref{cor:coverDownclosure}) implies
  $\downclosure {(\downclosure U \cap \downclosure{\SING{s}})}
    <|
  \downclosure V \cap\downclosure{(\downclosure U\cap \downclosure{\SING{s}})}$.

  Since we have
  $\downclosure{(\downclosure U \cap \downclosure V)}=\downclosure U \cap \downclosure V$,
  we can deduce that
  \[
    s
    \quad <| \quad
    \downclosure U \cap \downclosure {\SING{s}}
    \quad <| \quad
    \downclosure U \cap \downclosure V \cap \downclosure {\SING{s}}
    \quad\sub\quad
    \downclosure U \cap \downclosure V
    \ \hbox{.}
  \]
\end{proof}


However, strictly speaking, the proof of lemma~\ref{lem:convDistr} doesn't
apply to the preorder context. Instead, we have to match the operator
generated by adding the $\leq$-compat rule (\vpageref{compat-rule}), and
define:
\begin{defn}  \label{defn:convISClosure}
  if $<w,\leq>$ is an interaction structure with self simulation, we write
  $\A_{w,\leq}$ for the predicate transformer
  $\A_{w}(\downclosure U)$, where $\downclosure U$ is the downclosure of $U$,
  \ie~$\downclosure{U} == \{s\ |\ (\exists
  s'|= U)\, s\leq s'\}$.
\end{defn}
The intuition is quite straightforward: if $s'$ can simulate a state $s$
($s'\leq s$) in $U$, then $s'$ ``should'' be in $U$ as well. This is way to
say that our notion of simulation is semantically a real simulation.

\begin{cor}
  If $w$ is an interaction structure and $\leq$ a localized preorder on $S$;
  then the collection of open sets (\ie~the collection of $U$
  \st~$U=\A_{w,\leq}(U)$) is distributive.
\end{cor}


\paragraph{Computational interpretation.}

What have been done above is merely the result of transposing the definitions
from \cite{induc_top} in the context of interaction structures; but it was not
obvious how to make good computational sense of those. We present some of the
ideas now. The main point will be that to interpret localization, one needs to
move away from the Angel (client, $<|$ operator) perspective and take the
Demon (server, $|><$ operator) perspective.


\medbreak
For example, lemma~\ref{lem:localized} means that it is always possible for
the Angel to conduct interaction in such a way as to always simulate the
starting state; in particular, the Angel can make sure he can always ``change
his mind''.  An example of impossible command in such a system is
``\texttt{Initialize}'', a command which brings the whole system back to an
initial state. This will forget everything about past interactions, which is
impossible in a localized structure. Another, even more extreme, example is a
``\texttt{kill-self}''...

Thus, localization is a very strong condition on interaction structures;
especially if one has a ``games'' interpretation.

\begin{remark}
  Note that the notion of ``localization'' for a game is quite different from
  the notion of backtracking present in \cite{coquandGames} which allows to
  give a notion of games for classical logic.

  That the Angel is allowed to backtrack means that the Angel can ``go back in
  the past''. If the game is localized, then the Angel does not go back to a
  previous state, he can play in the current state, ``as if it were a previous
  state''. In particular, the Angel doesn't lose the possibility of doing the
  last available moves.
\end{remark}

\noindent
A second problem comes with the interpretation of the proof of
proposition~\ref{prop:localizedConvergent}: a non-canonical choice was made.
In the proof, we decided to first execute the client corresponding to $s <|
U$, and then the client corresponding to $s <| V$ on top of it. The opposite
works just as well:

\[
  s
  \quad <| \quad
  \downclosure V \cap \downclosure{\SING{s}}
  \quad <| \quad
  \downclosure V \cap \downclosure U \cap \downclosure{\SING{s}}
  \quad\sub\quad
  \downclosure V \cap \downclosure U
  \ \hbox{.}
\]
The two different witnesses for $s <| \downclosure U \cap \downclosure V$ may
be quite different in terms of execution! Here is what happens in graphical terms:
\begin{center}
  \input{./compose_localize.pstex_t}
\end{center}
On the left are the two client programs witnessing $s <| U$ and $s <| V$; and
on the right, the two different programs witnessing $s <| \downclosure
U\cap\downclosure V$.

Even worse, when the programs corresponding to $s <| U$ and $s <| V$ are
non-trivial, we could interleave the programs before reaching $\downclosure U
\cap \downclosure V$!


\bigbreak
A way to give (good) computational sense to the notion of localization is to
move away from the games intuition. The self-simulation $\geq$ will be seen as
a relation between ``internal'' states of the server and ``visible'' states
for the client(s). That this is a (general) simulation guarantees that we can
conduct interaction in the following way:
\begin{enumerate}
  \item if $s'\leq s$, \ie~the Angel thinks the Demon is in a state $s$, but
    internally, the Demon is really in a state $s'$;

  \item the Angel sends a request $a$ and receives an answer $d$;

  \item the Demon does the following:
    \begin{enumerate}
      \item translates the $a\in A(s)$ into a $a'\in\RTC{A}(s')$ (by
        simulation),
      \item responds to $a'$ with $d'\in \RTC{D}(s',a')$ (because it is a
        server program),
      \item and translate this answer $d'$ into a $d\in D(s,a)$ (by
        simulation),
    \end{enumerate}
    and gives this answer $d$ back to the Angel;

  \item the Angel now thinks the new state is $n(s,a,d)$ while internally, the
    Demon is really in state $\RTC{n}(s',a',d')\leq n(s,a,d)$;
\end{enumerate}
In particular, after the last point, the Angel can continue interaction.

\smallbreak
Localization can then be seen as the following requirement: suppose the Demon
is internally in a state $s$ and that there are two clients who respectively
think it is in state $s_1$ and $s_2$. The two clients can send their requests
and the Demon can answer to both of them (as above) in any order: suppose the
Demon starts by answering to the first client, then in point (a) in the above
interaction, the Demon can chose some $a'$ which always end in a state
$\RTC{n}(s',a',d')\leq n(s_1,a_1,d_1)$ (like above), so that the first client
can continue interaction \emph{and} $\RTC{n}(s',a',d')\leq s \leq s_2$ (by
localization). This last point guarantees that the server can now answer
requests to the second client...

In other words, localization simply means that we can construct ``concurrent
servers'' in the sense that several client may connect at the same time.

\medbreak
A good way to localize any interaction structure on $S$ is the following:
define $\L(w)$ on $\mathit{List}(S)$ as
\be
  \ISA{\L(w)}(l)         &==& \hbox{``}\SI{s |= l} \ISA{w}(s)\hbox{''}\\
  \ISD{\L(w)}(l,<s,a>)   &==& \ISD{w}(s,a)\\
  \ISn{\L(w)}(l,<s,a>,d) &==& l+s[a/d]
\ee
with the order $l\leq l'$ if ``every state in $l'$ is in $l$''. The
interaction structure $<\L(w),\leq>$ is localized.  The interpretation is
simply that the Demon keeps a log of all the previous states visited during
interaction, so that it can use any ``past'' state as the current one.

\begin{remark}
  To get a situation which is even closer to ``real life'', one can define a
  simulation $R : w -> \L(w)$ with $(s,l) |= R$ iff ``$s|= l$'' and use the
  extension from section~\ref{sec:extending} to interpret interaction...

  The idea is simply that we localize ``internally'' while still offer the
  services from the real interface: the clients are themselves not allowed to
  use those general states.
\end{remark}

\paragraph{Points.}

Now that the notion of localized interaction structure (aka formal topology)
has a computational interpretation, we can look (at last) at the notion of
formal point. A formal point in a formal topology on $S$ is a subset $\alpha
\sub S$ s.t.:
\begin{itemize}
  \item $\alpha$ is closed;
  \item $\alpha$ is convergent, \ie~$s|=\alpha$ and $s'|=\alpha$ imply that
    $s\BinDown s' \olp \alpha$.
\end{itemize}
We have already described the computational interpretation of a closed subset
in section~\ref{sec:clientServer}: the closed subset $\J(V)$ is given by a
server program which can maintain the invariant $V$.\footnote{It is
straightforward to extend the $\J$ operator to the case of interaction
structure with self simulations: $\J_{w,\leq}(V) = \J_w(\upclosure{V})$.}

\smallbreak
\noindent
Thus, a point is nothing more than a server program which satisfies
\begin{itemize}
  \item if $s_1 |= \alpha$ (a client may connect in state $s_1$)

  \item and if $s_2 |= \alpha$ (a client may connect in state $s_2$)

  \item then there is a(n internal) state $s$ which simulates both $s_1$ and
    $s_2$ (since $s|= s_1\BinDown s_2$) s.t. $s|=\alpha$. In other words,
    the server can find an internal state which will allow to respond to both
    $s_1$ and $s_2$.
\end{itemize}


Formal points are thus ``coherent'' server programs in the sense that they can
satisfy any finite number of ``unrelated'' concurrent clients.


\paragraph{Continuous maps.}

A relation $R$ between two localized interaction structure $w_h$ and $w_l$ is
called a continuous map if we have (see~\cite{BPIV}):
\begin{itemize}
  \item $R$ is a general simulation from $w_h$ to $w_l$;
  \item $R$ is total: $S_l <|_{w,\leq} R(S_1)$;
  \item $R(s_1)\BinDown R(s_2) <|_{w,\leq} R(s_1\BinDown s_2)$.
\end{itemize}
Similar interpretation can be devised for continuous maps as for formal
points, but the relevance of this interpretation in terms of actual
client/server programming is still unclear. We prefer to leave the matter open
for the time being.


%%% removed (old)  there are several technical things I am not totally sure about.
%%%         I added some blabla with the first mention of (.) in the
%%%         topological section.
%%%
%%% One final consequences of localization justifies our identification of the
%%% angelic tensor with the topological product.
%%% \begin{lem} \label{lem:AtensorProduct}
%%%   ``$\odot\!$'' is a coproduct in the category of localized interaction
%%%   structures with total\/\footnote{where a simulation $R:w_h->w_l$ is total if
%%%   $S_l <| R(S_h)$.} general simulations and equality up to saturation.
%%% \end{lem}
%%% \noindent
%%% So, if one passes to the dual category (\ie~the category of generated basic
%%% topologies), $\odot$ is a (categorical) cartesian product.  The proof is not
%%% difficult, and not very interesting from a computational point of view; we
%%% thus leave it open for the reader to investigate!
%%%
%%% More interestingly, the projections are ``really'' continuous in the sense
%%% that satisfy the additional condition of ``convergence'' (see~\cite{BPIV}).



==> rules.tex <==
\catcode`@=11
\let\ea=\expandafter

\def\tvi{\vrule height12pt depth5pt width0pt}

%%% a macro to typeset a rule of the form
%%%      h1   h2   h3    h4
%%%  ------------------------- name
%%%           conclu
%%%
%%% as \infer{h1&h2&h3&h4}{concl}{name}

\newbox\hyp \newbox\concl \newdimen\ruleWidth

\def\rule@nd{\rule@end}

%%% to insert space between the hypotheses
\def\rule@ux#1&{
 \def\tmp{#1}
  \ifx\tmp\rule@nd
   \hskip-2em$
    \else\tmp\hskip2em\ea\rule@ux
     \fi}

%%% the main macro
\def\infer#1#2#3{\relax
 \setbox\hyp=\hbox{$\rule@ux#1&\rule@end&} \setbox\concl=\hbox{$#2$}
  \ifdim \wd\concl<\wd\hyp
   \ruleWidth=\wd\hyp
    \else\ruleWidth=\wd\concl
     \fi
     \advance\ruleWidth by 1cm
     $\vcenter{
       \vbox{\hbox to\ruleWidth{\hss\tvi \unhbox\hyp \hss}}
        \hrule height.7pt depth0pt width\ruleWidth
         \vbox{\hbox to\ruleWidth{\hss\tvi \unhbox\concl \hss}}}$
          \kern.1cm \hbox{#3}}

\catcode`@=12

